Delaunay Component Analysis for Evaluation of Data Representations

Advanced representation learning techniques require reliable and general evaluation methods. Recently, several algorithms based on the common idea of geometric and topological analysis of a manifold approximated from the learned data representations have been proposed. In this work, we introduce Delaunay Component Analysis (DCA) - an evaluation algorithm which approximates the data manifold using a more suitable neighbourhood graph called Delaunay graph. This provides a reliable manifold estimation even for challenging geometric arrangements of representations such as clusters with varying shape and density as well as outliers, which is where existing methods often fail. Furthermore, we exploit the nature of Delaunay graphs and introduce a framework for assessing the quality of individual novel data representations. We experimentally validate the proposed DCA method on representations obtained from neural networks trained with contrastive objective, supervised and generative models, and demonstrate various use cases of our extended single point evaluation framework.

==> Sections/algorithms.tex <==

\begin{algorithm}
\caption{Delaunay Component Analysis} 
\begin{algorithmic}
\REQUIRE sets of representations $R$ and $E$
\REQUIRE number of sampled rays $T$
\REQUIRE sphere coverage parameter $B$
\REQUIRE minimum cluster size $mcs$
\REQUIRE component consistency threshold $\eta_c$ 
\REQUIRE component quality threshold $\eta_q$
\STATE \textbf{[Phase 1: Manifold approximation]}
\STATE $\mathcal{G}_D \gets \texttt{approximate_Delaunay_graph}(R, E| T)$
\IF{$B < 1.0$}
\STATE $\mathcal{G}_D \gets \texttt{filter_Delaunay_graph}(\mathcal{G}_D| B)$ (Section~\ref{sec:method-sphere-coverage})
\ENDIF
\STATE \textbf{[Phase 2: Manifold distillation]}
\STATE $\mathcal{G}_{DD} \gets \texttt{distil_Delaunay_graph}(\mathcal{G}_D| mcs)$ 
\STATE \textbf{[Phase 3: Manifold evaluation]}

\STATE \textbf{[Local evaluation]}
\STATE $\mathcal{C} \gets \texttt{get\_connected\_components}(\mathcal{G})$
\STATE $\mathcal{Q}_{\text{local}} \gets \texttt{zeros(len($\mathcal{C}$), 2)}$
\FOR{$i = 0, \dots, \texttt{len($\mathcal{C}$)}$}
\STATE $\mathcal{G}_i \gets \mathcal{C}[i]$
\STATE compute $c(\mathcal{G}_i)$ and $q(\mathcal{G}_i)$ as in Definition \ref{def:local_scores}
\STATE $\mathcal{Q}_{\text{local}}[i, :] \gets [c(\mathcal{G}_i), q(\mathcal{G}_i)]$
\ENDFOR
\STATE \textbf{[Global evaluation]}
\STATE compute $c(\mathcal{G}), q(\mathcal{G}), \mathcal{P}(\eta_c, \eta_q), \mathcal{R}(\eta_c, \eta_q)$ as in Definition \ref{def:global_scores}
\STATE $\mathcal{Q}_{\text{global}} \gets [\mathcal{P}, \mathcal{R},  c(\mathcal{G}), q(\mathcal{G})]$
\end{algorithmic}
\textbf{Return:} $\mathcal{Q}_{\text{global}}$, $\mathcal{Q}_{\text{local}}$
\label{alg:dca-alg}
\end{algorithm}


\begin{algorithm}[h]
    \caption{Delaunay Component Analysis}
    \label{alg:sph-int}
    \begin{algorithmic}    
    \Require sets of representations $R$ and $E$
    \Require number of sampled rays $T$
    %\Require sphere coverage parameter $B$
    %\Require minimum cluster size $mcs$
    %\Require component consistency threshold $\eta_c$ 
    %\Require component quality threshold $\eta_q$
    \State \textbf{[Phase 1: Manifold approximation]}
    \State $\mathcal{G}_D \gets \text{approximate\_Delaunay\_graph}(R, E| T)$
        % $\Sigma \subset \mathbb{S}^{n-1}$ set of $r$ versors
        % \Ensure $\vol_p$ for all $p\in P$
        \State Compute $(q, p) \in P \times P$
        % \State Compute $\inner{\sigma}{p}$ \kw{for all} $(\sigma, p) \in \Sigma \times P$
        % \ForAll{$p \in P$}
        %     \State Initialize $\vol_p \leftarrow 0$
        %     \ForAll{$\sigma \in \Sigma$}
        %         \State Initialize $l_p(\sigma) \leftarrow \infty$
        %         \ForAll{$q \in P \setminus \{p\}$}
        %             \State $l^q_p(\sigma)) \leftarrow \frac{\inner{q}{q} - 2\inner{q}{p} + \inner{p}{p}}{2\inner{\sigma}{q} - 2\inner{\sigma}{p}}$
        %             \If{$l^q_p(\sigma)) > 0$}
        %                 \State $l_p(\sigma) \leftarrow \text{min}\{ l_p(\sigma), l^q_p(\sigma) \}$
        %             \EndIf
        %         \EndFor
        %         \State $\vol_p \leftarrow \vol_p + \frac{\left(2\pi h^2\right)^{\frac{n}{2}}}{r} \overline{\gamma}\left(\frac{n}{2}, \ l_p(\sigma)\right)$
        %     \EndFor
        % \EndFor
    \end{algorithmic}
\end{algorithm}

==> Sections/old_experiments.tex <==


\noindent \textbf{Cluster assignments} We proceed with applying our q-DCA algorithm, presented in Section~\ref{sec:method-extension}, to analyze the robustness of the SimCLR model to novel images not seen during the training. For this, we constructed three different query sets: $Q_1$ and $Q_2$ each containing $50$ test representations of classes $c_0, \dots, c_6$ not used in $E$ and $c_7, \dots, c_{11}$, respectively, and $Q_3$ comprising of $250$ randomly chosen representations of images of all classes that were recorded from the right camera view (see Figure~\ref{fig:boxes}). To eliminate effects of data imbalances, $R$ and $E$ contained exactly $250$ representations from each of the $7$ classes $c_i$. By construction, we expected $Q_1$ to be close to existing fundamental connected components in the distiled Delaunay graph $\mathcal{G} = \mathcal{G}_{DD}(R \cup E)$ and $Q_2$ further away. Moreover, if SimCLR is robust to the semantic content in the right-view images, points in $Q_3$ labeled with first $7$ classes are expected to be close to $\mathcal{G}$, while the remaining ones should lie further apart.

\begin{comment}
%Using our q-DCA algorithm presented in Section~\ref{sec:method-extension}, we additionally analyzed the robustness of the SimCLR model to novel images not seen during the training. 
For this, we constructed balanced $R$ and $E_6$ sets %from $\mathcal{D}_f^R$ and $\mathcal{D}_f^E$, respectively, 
by randomly sampling exactly $250$ representations from each of the $7$ classes $c_i$. We then sampled $50$ more representations of classes $c_0, \dots, c_6$ that were not used in $E$ to construct the set of query representations $Q_1$,
%images encodings from $\mathcal{D}_f^E$ that were not used in $E$ from each of the classes $c_0, \dots, c_6$ to construct $N_1$, 
and of classes $c_7, \dots, c_{11}$ to construct $Q_2$. Lastly, we constructed $Q_3$ by randomly sampling $250$ representations of images of all classes that were recorded from the right camera view (see Figure {\orange X}). Therefore, the representations in $Q_1$ should be close to existing connected components in the distiled Delaunay graph $\mathcal{G}(R \cup E_6)$, while those in $Q_2$ should lie further away. Moreover, if SimCLR is robust to semantic content in the novel images, the representations in $Q_3$ corresponding to first $7$ classes should lie close to $R$ or $E_6$ as they represent the same box configuration but recorded from different camera view, while the remaining ones should lie further apart.
\end{comment}

To obtain an assignment (if any) of a query point $z_j \in Q_k$ to an existing fundamental component $\mathcal{G}_f = (\mathcal{V}^{\mathcal{G}_f}, \mathcal{E}^{\mathcal{G}_f}) \in \mathcal{F}$,  we analyzed the edges inserted using q-DCA. Recall that due to the nature of Delaunay graphs, $z_j$ can have edges associated to several $\mathcal{G}_f$ although these vary in their length. Therefore, we considered only those inserted edges whose length were representative of the connected components they connected to, i.e, we calculated the mean $\mu(\mathcal{E}^{\mathcal{G}_f})$ and std $\sigma(\mathcal{E}^{\mathcal{G}_f})$ of the length of edges in each $\mathcal{G}_f \in \mathcal{F}$ and kept only edges in $N(z_j) \cap \mathcal{G}_f$ that were shorted than $\mu(\mathcal{E}^{\mathcal{G}_f}) + \sigma(\mathcal{E}^{\mathcal{G}_f})$. We refer to these edges as \textit{typical edges} and define two assignment procedures: (1) \textit{conservative} where we assigned $z_j$ to a component $\mathcal{G}_f$ only if all typical edges connected $z_j$ to exactly one $\mathcal{G}_f$ and did not assign it to any otherwise, and (2) \textit{flexible} where we additionally assigned $z_j$, whose typical edges connected to more than one component, to a component $\mathcal{G}_f$ if it attained both shortest and max number of typical edges among all the candidate components. 

%We applied q-DCA version $3$ to obtain assignments (if any) of representations in each of the constructed $Q_k$ to an existing connected component in $\mathcal{G}$. For this, we calculated the mean $\mu(\mathcal{G}_i^F)$ and standard deviation $\sigma(\mathcal{G}_i^F)$ of Delaunay edges contained in fundamental connected components $\mathcal{G}_i^F$ {\orange Fix Notation}. For each novel point $z_j \in N_k$, we extracted the number of novel edges $n_{j, i}$ between $z_j$ and each $\mathcal{G}_i^F$  as well as the length $L_{j, i}$ of the shortest edge among them. Due to the nature of Delaunay graphs, each point $z_j$ can have edges associated to several connected components although these vary in their length. We therefore further extracted only those edges whose lengths were representative of the connected components they connected to, i.e., we kept the statistics of $z_j$ and $\mathcal{G}_i^F$ if only if $L_{j, i} \le \mu(\mathcal{G}_i^F) + \sigma(\mathcal{G}_i^F)$. We refer to the later condition as \textit{assignment condition}. We defined two assignment procedures: (1) \textit{conservative} where we assigned a point $z_j$ to a component $\mathcal{G}_i$ only if the assignment condition holds for exactly one $\mathcal{G}_i^F$ and do not assign it to any otherwise, and (2) \textit{flexible} where we additionally assigned a point $z_j$, whose assignment condition holds for more than one connected component, to a component $\mathcal{G}_i^F$ if it attains both shortest edge $L_{j, i}$ and max number of edges $n_{j, i}$ among all the candidate components. 

Using class labels $c_i$, we first determined the majority-vote label of each $\mathcal{G}_f$ (which we observed to be almost perfect). Given the labels of $z_j \in Q_k$, 
%We then we extracted representations from $Q_k$ that 
we then extracted those $z_j$ that \textit{(a)} should be assigned to a component and report the percentage $A$ of them that were assigned to the one with the same label, %: $\%$ \textit{should be assigned}, 
and \textit{(b)} that were assigned and report the percentage $B$ of those that were correctly assigned. %: $\%$ \textit{were assigned}. 
Thus, for $Q_1$, the extracted representations in \textit{(a)} is the entire set $Q_1$. Same holds for $Q_2$ as in this case we assumed that points in $Q_2$ should not be assigned to any component and thus report the percentage of those that were correctly not assigned to any.
%Thus, for $Q_1$, the extracted representations in (a) is the entire set $N_1$. The same holds for $N_2$ as in this case we assumed that points in $N_2$ should not be assigned to any component and thus report the percentage of those that were correctly not assigned to any. 
In $Q_3$, we consider a combination of the two cases, where $1750$ representations corresponding to $c_0, \dots, c_6$ should be assigned to a component if the model is able to extract the underlying semantic information, while the remaining $1250$ representations corresponding to $c_i, i \ge 7$  should not. Therefore, for all $Q_i$, the higher $A$ the better. For $B$, the higher the better for $Q_1$, while for $Q_2$ and $Q_3$ it holds that the lower the better.
%$\%$ \textit{should be assigned} the better. For  $\%$ \textit{were assigned}, the higher the better for $N_1$, while for $N_2$ and $N_3$ it holds that the lower the better.


%Using ground truth class labels, we extracted representations that should be assigned to a component (e.g., representations of class $c_2$ in $N_1$) and report the percentage of those that were assigned to the correct component: $X_{should\_be\_assigned}$. Note that in case of representations whose class labels $c_i > 6$, we extract representations that should not be assigned to any component and report the percentage of those that correctly were not assigned to any. Secondly, we extract all the representations that were (not) assigned and report the percentage of those that were (not) correctly assigned $X_{were\_assigned}$.  


\begin{table}[h]
\caption{Results of assignments of points in query sets $Q_k$ to fundamental components $\mathcal{G}_f \in \mathcal{F}$.}
\label{tab:cluster-assignment}
\begin{center}
\begin{tabular}{c|ccc|ccc}
                                  & \multicolumn{3}{c|}{A = \% that should be assigned  } & \multicolumn{3}{c}{B = \% that were assigned}  \\
                                  & $Q_1 (\uparrow)$ & $Q_2 (\uparrow)$ & $Q_3 (\uparrow)$               & $Q_1 (\uparrow)$ & $Q_2 (\downarrow)$ & $Q_3 (\downarrow)$        \\ 
\hline\hline
\multicolumn{1}{r|}{conservative} & $0.62$ & $0.69$ & $0.28$               & $1.00$ & $0.00$ & $0.08$        \\
\multicolumn{1}{r|}{flexible}     & $0.99$ & $0.66$ & $0.16$               & $1.00$  & $0.00$  & $0.08$       
\end{tabular}
\end{center}
\end{table}


We show the assignment results in Table~\ref{tab:cluster-assignment}. For $Q_1$, we see that the conservative approach resulted in $A = 62\%$ and $B = 100\%$.
%of the points that should be assigned and all the points that were assigned being correctly assigned. 
The former is due to the fact that $133$ representations out of $350$ are assigned to several components. Of out these, $129$ points were considered in the flexible assignment yielding an increase of $A$ %$\%$ \textit{should be assigned} 
to $99\%$ of correct assignments. 
For $Q_2$, the conservative approach resulted in $A = 69\%$ due to $78$ points being assigned to a component despite their wrong label $c_i, i \ge 7$ (thus leading to $B = 0 \%$). This suggests that classes are moderately separated in the representation space, which is on par with the analysis performed by~\cite{geomca} who showed that SimCLR achieves worse class separation than the compared alternatives.
%For $N_2$, the conservative approach resulted in $69\%$ of the points that should be not assigned being correctly not assigned to any component. None of the $78$ points that were assigned to a component were correctly assigned as these are labeled with $c_i, i \ge 7$. 
%Due to a portion of representations being wrongly assigned, we conclude that the classes are moderately separated in the representation space. This conclusion is on par with the analysis performed by~\cite{geomca}, who showed that the SimCLR model achieves worse class separation. {\orange compared to alternative models.}
For $Q_3$, we see that $A = 28 \%$ and $B = 8\%$ in the conservative approach which indicates that SimCLR is not able to recognize similar box configurations recorded from different camera view, which is aligned with the results obtained by~\cite{chamzas2021comparing}. Lastly, we observe that flexible approach yielded only minor decrease in $A$ for $Q_2$ and $Q_3$. 
%For $N_3$, we see that in the conservative approach, only $28 \%$ of points that should be assigned and only $8\%$ of those that were assigned were in fact correctly assigned. This shows that SimCLR model is not able to recognize similar box configurations recoded from different camera view, which is aligned with the results obtained by {\orange CITE MM}.


